Polar Ring Galaxies in the Galaxy Zoo

We report observations of 16 candidate polar ring galaxies (PRGs) identified by the Galaxy Zoo project in the Sloan Digital Sky Survey (SDSS) database. Deep images of five galaxies are available in the SDSS Stripe82 database, while to reach similar depth we observed the remaining galaxies with the 1.8-m Vatican Advanced Technology Telescope. We derive integrated magnitudes and u-r colours for the host and ring components and show continuum-subtracted H\alpha+[NII] images for seven objects. We present a basic morphological and environmental analysis of the galaxies and discuss their properties in comparison with other types of early-type galaxies. Follow-up photometric and spectroscopic observations will allow a kinematic confirmation of the nature of these systems and a more detailed analysis of their stellar populations.

==> proof <==
Q1 - OK
Q2 - OK
Q3 - OK
Q4 - OK
Q5 - OK
Q6 - OK
Q7 - please replace right panel of Fig. 4 with the attached file (PRGlc.eps)
Q8 - This acronym is commonly used and a reference is given.
Q9 - The expression is OK.
Q10 - please add to the reference list: 'Bekki  K., 1997, ApJ, 490, 37'
Q11 - OK
Q12 - please add to the reference list: 'Schawinski K. et al., 2009, MNRAS, 396, 818'.
Q13 - please replace 'Dr. Jonathan Stott' with  'Jonathan Stott S.J.'.
Q14 - this is the reference generally given in MNRAS papers.
Q15 - please remove from the reference list
Q16 - please remove from the reference list
Q17,18 - Please replace 'Kavirag' with 'Kaviraj', more than eight authors, no update
Q19 - please update 'Moiseev A., Smirnova K., Smirnova A., Reshetnikov V., 2011, MNRAS, 418, 244'.
Q20,21 - please remove from the reference list.
Q22 - no update.
Q23,24 - please remove from the reference list.


More comments:

Page 1, second column, line 45: add at the end of the sentence Lintott et al. 2008 as follows: '...answer a standard set of questions about their features.'  -> '...answer a standard set of questions about their features (Lintott et al. 2008).'
Add to the reference reference 'Lintott C.J.\ et al., 2008, MNRAS, 389, 1179'

Page 1, second column, line 53-54: replace 'for selecting newnearby candidate PRG from the Galaxy Zoo.' with 'for selecting newnearby candidate PRGs from the Galaxy Zoo.' ('PRG' -> 'PRGs')

In Table 3, third column, last row (D-ETGs/Unclassified): replace '28 per cent' with '6 per cent'

